Towards the classification of rank-$r$ $\mathcal{N}=2$ SCFTs. Part I: twisted partition function and central charge formulae

We derive explicit formulae to compute the $a$ and $c$ central charges of four dimensional $\mathcal{N}=2$ superconformal field theories (SCFTs) directly from Coulomb branch related quantities. The formulae apply at arbitrary rank. We also discover general properties of the low-energy limit behavior of the flavor symmetry of $\mathcal{N}=2$ SCFTs which culminate with our $\mathcal{N}=2$ UV-IR simple flavor condition. This is done by determining precisely the relation between the integrand of the partition function of the topologically twisted version of the 4d $\mathcal{N}=2$ SCFTs and the singular locus of their Coulomb branches. The techniques developed here are extensively applied to many rank-2 SCFTs, including new ones, in a companion paper.

==> S3_higher_ranks.tex <==
\section{Higher ranks}

In this case the stratification of the is more involved and higher complex codimension strata appear. Thus some might think that the deformation pattern which played a prominent role in defining what we meant by the \emph{physical discriminant}, might have to be further enriched by other information.  

We instead claim that both the $\cB$ and the $\cC$ factor only get contributions from the complex co-dimension one singular loci which support theory of rank-1, and therefore even this case, the dependence of the partition of the topologically twisted theory, can be characterized by the \emph{physical} discriminant which is largely analogous to what we discussed above. In fact the two holomorphic pieces appearing in the partition function will have the following form:
\begin{align}
\cB(\bu)=\prod_{i=1}^\nf P_i(\bu)^{b_i}\\
\cC(\bu)=...
\end{align} 
next we perform a few checks on Lagrangian theories, higher rank F-theory constructions as well as AD theories of rank-3, that this indeed works. 


\red{also possibly add a remark about the fact that all the mass deformations split the asymptotics of the CB and therefore are visible by the splitting of the complex co-dimension one part of the singular locus. This is an encouraging result that the systematic study of mass deformations of higher rank theory can indeed be reduced ultimately to a problem of studying mass deformations of rank-1 theories and therefore there is a way to generalize the analysis of \cite{Argyres:2015ffa,Argyres:2015gha,Argyres:2016xua,Argyres:2016xmc} to study these cases.}

\subsection{Checks}

\subsubsection{$SU(4)$ with $N_f=8$}

\subsubsection{$SU(4)$ with $N_f=8$}

\subsubsection{$SU(4)$ with $N_f=8$} 
